On the Relationship Between Explanation and Prediction: A Causal View

Being able to provide explanations for a model's decision has become a central requirement for the development, deployment, and adoption of machine learning models. However, we are yet to understand what explanation methods can and cannot do. How do upstream factors such as data, model prediction, hyperparameters, and random initialization influence downstream explanations? While previous work raised concerns that explanations (E) may have little relationship with the prediction (Y), there is a lack of conclusive study to quantify this relationship. Our work borrows tools from causal inference to systematically assay this relationship. More specifically, we study the relationship between E and Y by measuring the treatment effect when intervening on their causal ancestors, i.e., on hyperparameters and inputs used to generate saliency-based Es or Ys. Our results suggest that the relationships between E and Y is far from ideal. In fact, the gap between 'ideal' case only increase in higher-performing models -- models that are likely to be deployed. Our work is a promising first step towards providing a quantitative measure of the relationship between E and Y, which could also inform the future development of methods for E with a quantitative metric.

==> _preamble/packages.tex <==
\usepackage{arabtex}
\usepackage[utf8]{inputenc}
% \usepackage{utf8}
\setcode{utf8}

\usepackage{lipsum}
\usepackage{color, soul}
% \usepackage[colorlinks=true, linkcolor=red, urlcolor=blue, citecolor=blue, anchorcolor=blue]{hyperref}
% \usepackage[numbers, sort, compress]{natbib}
\usepackage{bibentry}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{amsmath,amsthm,amssymb} % error: https://pctex.com/kb/86.html
\usepackage{mathtools}
% \usepackage[algoruled,vlined,nofillcomment]{algorithm2e}
\usepackage{listings}
\usepackage{multirow}
\usepackage{hhline}
\usepackage{changepage} % used for adjustwidth (for large tables)
\usepackage{adjustbox}
% \usepackage{subcaption} % subfigure is obsolete and doesn't work with listings; using subcaption instead
\usepackage{url}
\usepackage{wrapfig}
\usepackage{booktabs}
\usepackage{siunitx}
% \usepackage{unicode-math} % does not work with pdflatex
% \setmathfont{xits-Math}

% https://tex.stackexchange.com/a/58684
\usepackage{caption}
\captionsetup[table]{skip=3pt}

% \usepackage{colortbl} % https://stackoverflow.com/a/57222641
% \usepackage[table]{xcolor} % https://tex.stackexchange.com/a/5365
% \PassOptionsToPackage{table}{xcolor, }

\usepackage{tabularx}

% https://tex.stackexchange.com/a/129960
\usepackage{enumitem}

% https://tex.stackexchange.com/a/118955
% https://ctan.mc1.root.project-creative.net/fonts/fontawesome/doc/fontawesome.pdf
\usepackage{fontawesome}

\usepackage{fetamont} % Used for ffmfamily below.
\usepackage[T1]{fontenc} % Used for ffmfamily below.

\usepackage{centernot}
\usepackage[final]{pdfpages}

\usepackage{thmtools, thm-restate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin NeurIPS paper
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{nccmath}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{tikz}
\usetikzlibrary{bayesnet}
% \usepackage{subcaption}
\usepackage{tabularx}
\usepackage{mathtools}
% \usepackage{cleveref}
\usepackage{thmtools, thm-restate}
\usepackage{multirow}
\usepackage{changepage} % used for adjustwidth (for large tables)
\usepackage{adjustbox} % used to place tikzpicture inside tabular cell
\usepackage{lipsum}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End NeurIPS paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin MACE* paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amsmath}
% \usepackage{subfiles}
\usepackage[framemethod=tikz]{mdframed}
\usepackage{tikz}
\usepackage{footmisc}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End MACE* paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin Robust Recourse paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
% \usepackage{subfigure}
\usepackage{booktabs} % for professional tables

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2022} with \usepackage[nohyperref]{icml2022} above.
\usepackage{hyperref}


\usepackage{xcolor}
\definecolor{def1}{rgb}{0.12, 0.47, 0.705}
\definecolor{def2}{rgb}{1.0, 0.5, 0.055}
\definecolor{def3}{rgb}{0.17, 0.63, 0.17}
\definecolor{def4}{rgb}{0.84, 0.15, 0.16}
\definecolor{def5}{rgb}{0.58, 0.4, 0.74}
\definecolor{def6}{rgb}{0.74, 0.74, 0.13}
\DeclareRobustCommand{\legendsquare}[1]{%
  \textcolor{#1}{\rule{1.2ex}{1.2ex}}%
}
\newcommand{\tikzcircle}[2][black,fill=black]{\tikz[baseline=-0.5ex]\draw[#1,radius=#2] (0,0) circle ;}%

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2022}

% If accepted, instead use the following line for the camera-ready submission:
% \usepackage[accepted]{icml2022}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage[hidelinks]{hyperref}       % hyperlinks
% \usepackage{hyperref}
\hypersetup{hidelinks}
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{tabularx}
\usepackage{caption}
% \usepackage[export]{adjustbox}% http://ctan.org/pkg/adjustbox
\usepackage{dashbox}
%\usepackage[english]{babel}
% \usepackage{blindtext}
% \usepackage{subcaption}
% \usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{stackengine}
\usepackage{graphbox}
\usepackage{multicol}
\usepackage{float}

\newsavebox\CBox
\def\textBF#1{\sbox\CBox{#1}\resizebox{\wd\CBox}{\ht\CBox}{\textbf{#1}}}
% \parindent=0pt

\usepackage{tikz}
\usetikzlibrary{shapes,arrows,positioning}

% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}
% \newtheorem{theorem}{Theorem}
% \newtheorem{corollary}{Corollary}
% \newtheorem{lemma}{Lemma}
\newcommand\innerr[1]{\langle #1 \rangle} % TODO(amirhkarimi): fix conflict with \inner in commands.tex
\usepackage{makecell}
\usepackage{centernot}
\usepackage{makecell}

\renewcommand\theadalign{bc}
\renewcommand\theadfont{\bfseries}
\renewcommand\theadgape{\Gape[4pt]}
\renewcommand\cellgape{\Gape[4pt]}

\usepackage{bbm}
\usepackage{enumitem}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End Robust Recourse paper.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> _sections/011_related_work.tex <==

%1. other work that examined relationships between E and Y (e.g., sanity check, rethinking gradient) or just suspicious of explanations in general (we can carefully and briefly include robustness tests).

%~\cite{poursabzi2018manipulating,chu2020visual,adebayo2018sanity,alqaraawi2020evaluating,srinivas2021rethinking}. 

%Weights, hyperparams and performance\cite{Eilertsen2020, unterthiner2020predicting}

%2. counterfactual explanations vs what we are doing

%\been{copy from intro}

Although the treatment effects are identifable, evaluating them is computationally expensive.
%
To understand why, it helps to illustrate a parallel with the setting of counterfactual explanations~\citep{wachter2017counterfactual}.
%
Whereas the treatment effects in our setting (see \Cref{eq:ite}) contrasts $Y^*_{h}(x)$ and $Y^*_{h'}(x)$, the work of \citet{wachter2017counterfactual} contrasts $Y^*_{h}(x)$ and $Y^*_{h}(x')$.
%
Unlike the latter which only requires the invocation of the \emph{predicting procedure} given a new \instance~(e.g., a forward pass through a neural network), the former invokes the \emph{training procedure} given a new \hparam~setting (i.e., a full re-training).
%
In practice, computing power is limited and we may only have access to the predictions under a single model, say, $Y^*_{h}(x)$ and it can be prohibitively expensive to produce the prediction under a different model, $Y^*_{h'}(x)$, especially for large neural networks.


%\been{For Krik, also add this paper (commented)}% https://hastie.su.domains/Papers/pdp_zhao.pdf
%3.  causal inference work with high-dimension (e.g., causal embeddings?) to compare with our distributional treatement effect


In this work, we adopt the kernel treatment effect (KTE) to quantify the treatment effect of hyperparameters on prediction and explanation. Compared to the standard framework for univariate outcomes \citep{imbens2004nonparametric,rubin2005causal}, KTE enables us not only to work with the high-dimensional multivariate outcomes through positive definite kernels, but also to capture subtle effects of the hyperparameters on prediction and explanation that are beyond the mean effect; see, e.g., \citep{Muandet20:CME,singh2020kernel,Park21:CoDiTE} for detailed exposition.
Note that \citet{zhao2021causal} also aims to provide a causal interpretation of the black-box model using partial dependence plot (PDP). The authors observe that the formulation of PDP is exactly the same as the back-door adjustment formula of \citet{pearl2009causality}.
Although this work might be applicable to analyze the causal effects of interest in this work, the authors emphasize that it should not replace a random experiment or a carefully designed observational study.\km{I looked at the paper. Although the connection is not so clear, I tried to write something here. It would be great if someone could double check.}





==> _sections/_dep_010_introduction.tex <==


% NOTE: I wrote E and Y for convenience, but in real intro, I'll replaced them w/ more readable English.
% 1. explanations are important, lots of work done.
% 2. But also lots of questions are raised (eg sanity check paper, suraj's work) that hint that we don't really understanding relationship between E and Y. Why does this matter? Supposedly, E is explaining the rational behind the model's decision, Y, and not something else. But one may also argue that data distribution itself (eg good features from images) must also play a role in E, therefore, E may contain something beyond Y alone.
% 3. This paper is not about taking either side of that discussion, instead, our goal is to report a results from investigating relationship between E and Y, leveraging potential outcome framework.
% Specifically, we conduct observation study by computing treatment (hyper parameters) effect on E and Y. Here we are treating hyper parameters as different "environment" that we use to observe how E and Y's behavior changes. 
% 3.1 - add "why hyperparams?" Amir's paragraph below "A careful study..."
% 3.2 add paragraph on "viewed thru a lens of causality..." below on how to view hyper params as treatment effect.
% 4. Our analysis suggests that there is no correlated behavior between E and Y when we consider 30k models with different hyperparameters/environments. Even when we subdivide the population into similarly performing models, there is no trend both in terms of correlation or ranked correlations.
% [write more about our findings]
% 5. Our discussion helps practitioners who use interpretability methods for a concrete task (e.g., debugging). Knowing the lack of relationships between E and Y can inform them when these explanations can and cannot be used for. 



%1. explanations are important, lots of work done. GDPR.

Being able to provide explanations for a machine learning (ML) model's decision has become one of the central to developing, deploying and adopting ML models. 
Explanations are important not only to help practitioners better understand the model's underlying rationale to debug models~\citep{adebayo2020,Rieger2020InterpretationsAU} and to influence model's decision~\citep{koh2020concept,Bau2020,meng2022locating}, but also to ensure that models comply with regulatory requirements~\citep{gdpr16}.
% Active developments of interpretability tools was at the same time accompanied by pointed criticisms thereof
%Although ML researchers have developed many interpretability tools, these tools have elicited pointed criticisms, often highlighting computational or qualitative user-study-based evidence that explanations generated from these tools must be used with care~\citep{poursabzi2018manipulating,chu2020visual,adebayo2018sanity,alqaraawi2020evaluating,srinivas2021rethinking, kindermans2019reliability}. 
Existing tools for interpretability have, however elicited criticisms, often highlighting computational or qualitative user-study-based evidence that explanations generated from these tools may contain critical errors and must be used with care~\citep{poursabzi2018manipulating,chu2020visual,adebayo2018sanity,alqaraawi2020evaluating,srinivas2021rethinking, kindermans2019reliability}. 

%2. But also lots of questions are raised (eg sanity check paper, suraj's work) that hint that we don't really understanding relationship between E and Y. Why does this matter? Supposedly, E is explaining the rational behind the model's decision, Y, and not something else. But one may also argue that data distribution itself (eg good features from images) must also play a role in E, therefore, E may contain something beyond Y alone.

In particular, the relationship between explanations ($E$) and predictions ($Y$) has been one of the focal points in many investigations. Some studies argue that since many explanation methods claim to reveal a model's rationale behind its \textit{decision} ($Y$), there must be a ``strong correlation'' between $E$ and $Y$, e.g., when $Y$ changes significantly, $E$ must do so as well \cite{adebayo2018sanity,srinivas2021rethinking},
%\bernhard{the part after e.g. seems too restrictive, since $E$ can be high-dimensional and $Y$ scalar. Would it make sense the other way round?}\bk{the other way won't work but I'll edit a bit.}
while others argue that $E$ should also reflect other factors in addition to $Y$ such as features in data points and data distribution~\citep{adebayo2018sanity, nie2018theoretical, srinivas2021rethinking, bilodeau2022impossibility}. % $E$ is function of $Y$, $X$ and other factors). 
%
On the one hand, it has been observed empirically that explanations from an untrained model and a trained model can be visually and statistically indistinguishable~\citep{adebayo2018sanity}.
%
On the other hand, it was proven theoretically that $E$ has no relation to $Y$ in some cases  \citep{nie2018theoretical, srinivas2021rethinking}. However, quantitatively validating the relationship between $E$ and $Y$ while controlling for potential confounding factors such as hyperparameters and datasets remains an open question. 

%Intuitively speaking, 
%by defining functions generating $Y$ and $E$, and the correlation\bernhard{not sure I understood the bit about correlation --- maybe it's enough to directly jump to the treatment effect} of the two as a result (i.e., the difference in treatment effect of a causal ancestor
%\bernhard{could also say causal ancestor} 
%on $Y$ and $E$).\%bk{first take on the definition of the relationship. Feel free to edit}
%\bernhard{Maybe one could argue based on Reichenbach's principle here: By the common cause principle of \citep{Reichenbach1956}, whenever we find two variables to be dependent, there must be a common cause influencing both of them (and this common cause can be chosen such that it explains all the dependence). Below, we will take inspiration from this view on dependence, and develop a measure of dependence based on causal effects on our two quantities of interest, $Y$ and $E$. (Maybe we could give some argument why causal is better than just statistical here?)}\bk{I like this!}
%\bernhard{I think it would be good to somewhere (maybe here) clearly state what we mean by relationship between E and Y. How would such a relationship look? Do we think of them as random variables?}\bk{agreed! flag - we use this relationship informally but define quantify relationship.}

%\been{MMD-like functions generating Y and E are correlated}

%3. This paper is not about taking either side of that discussion, instead, our goal is to report a results from investigating relationship between E and Y, leveraging potential outcome framework. Specifically, we conduct observation study by computing treatment (hyper parameters) effect on E and Y. Here we are treating hyper parameters as different "environment" that we use to observe how E and Y's behavior changes. 

\input{_sections/pipeline_detail} 

%We will provide a formalization of this relationship below, but essentially we evoke
In this work, we seek to formalize this relationship, inspired by the common cause principle of \citet{Reichenbach1956} that states that if 
%, where we find 
two variables are {\em statistically} dependent, there must be a common {\em cause} influencing both of them, and this common cause can be chosen such that it explains all the dependence. 
We 
%will take inspiration from this view on dependence, and 
develop a measure of dependence %based on causal effects on our two quantities of interest, $Y$ and $E$ 
%In this work, we provide first steps towards quantifying factors that influence $E$ 
via the Potential Outcomes framework~\citep{rubin2005causal}. Viewed through a lens of causality, we evaluate the treatment effect of hyperparameters of the model, $H$ (i.e., $H$ taking on value $h'$, the counterfactual antecedent) on $E$ and $Y$ conditioned on a particular instance $x$. 
%We do this by conducting an observational study made possible by a large dataset of pre-trained models. 
%Viewed through a lens of causality, the counterfactual antecedent (i.e., $H$ taking on value $h'$) is a hypothetical intervention whose effect we want to measure on the target explanation, conditioned on a particular instance, $x$.
%, or subspace of the dataset, $\mathcal{X}' \subseteq \mathcal{X}$. %(e.g., all dog images). 
%\been{Amir: we actually use all classes and not just one class-dog-right? perhaps we can remove the e.g., to avoid confusion?} \amir{yes, let's remove; we may consider keeping the ATE/CATE definitions for completeness, but not necessary.}
In other words, by measuring the treatment effect of each hyperparameter (e.g., choice of activation, initialization, training budget), we are measuring its influence on $E$ and $Y$, and in particular, how the influence is \textit{different or similar} in $E$ and $Y$ (Fig.~\ref{fig:pipeline}; left). 
%
Furthermore, under a careful evaluation, we tease apart the direct influence of $H$ on $E$ vs. its indirect influence mediated through $Y$ to better understand the flow of causation (Fig.~\ref{fig:pipeline}; right).

%However, 
Note that we may not be able to interpret the observed differences between $Y$ and $E$ that arise from two different $H$ as a causal effect unless the assumption of \emph{ceteris paribus}, i.e., all else being equal, is fulfilled. Retraining almost identical neural networks with all possible values of hyperparameters is however computationally prohibitive. Instead, we perform an observational study on a model zoo, a large collection of pre-trained models \citep{unterthiner2020predicting, jiang2018predicting}, to
%verify our hypothesis on
study the relationship between $E$ and $Y$.%\km{How about this?}



Why hyperparameters as treatments? Under a fixed random seed, hyperparameters are arguably the only reasonable causal ancestor of the model because they fully determine the weights of the resulting model and behavior thereof.
%\been{Trying to say that this is kind of our only option, but please edit this to some better wordings}\amir{i added a bit; how's that? (accepted your changes from earlier so you can track mine)}
%Two potentially completely different models (thus, different rationale) can be trained with the same hyperparameters but different initialization (e.g., one of the stuck in local minima), 
%are widely studied in ML as one of prime factors that 
They are also known to influence the inherent tendencies/performances of the model. 
%3.1 - add "why hyperparams?" Amir's paragraph below "A careful study of the factors that play a role in generating outcomes is warranted, not just for XAI, but more generally in ML. 
For example, models trained on completely different hyperparameters could perform similarly under one metric (e.g., training loss), but have completely different task-specific performance, e.g., fairness~\citep{d2020underspecification}. 
One can also use the hyperparameters alone to predict the final performance of the models~\citep{unterthiner2020predicting} or even use model's weights to predict hyperparameters~\citep{Eilertsen2020}.
%\been{I recall there was work that just use hyperparams to predict performance too but can't locate it.}\amir{were you thinking of the model zoo paper itself \url{https://arxiv.org/abs/2002.11448}?}
%\been{ah maybe!}
% which may be attributed to the seemingly benign but consequential randomization seed.
%In the XAI literature specifically, prior work has shown that various saliency-based methods are independent of both the model and the underlying data, rendering the method unreliable~\citep{adebayo2018sanity, kindermans2019reliability}."

%3.2 add paragraph how to view hyper params as treatment effect from Amir's paragraph below:

Despite some methodological similarities, our work is fundamentally different from using causal inference to \textit{generate} 
%Our way of using hyper-parameter as an intervention can be seen as an interesting counterpart to the 
counterfactual explanations, e.g., \citet{wachter2017counterfactual},
where intervention is on the subset of features in an instance, rather than 
%which aims to identify a subset of features in an instance that would change the prediction of a fixed model. %by measuring treatment effects.
%In contrast, our work intervenes 
on a causal ancestor of $E$ while keeping the dataset constant. Our goal is to
%identify causal effect of $Y$ to $E$.
study the relation between $Y$ and $E$, and not to generate explanations.
%minimal feature perturbations of the dataset \instance~under a fixed model to flip the prediction (i.e., \hparams~do not change; procedure: \emph{model prediction}), evaluating treatment effects as the difference between counterfactual contrasts is done to identify \tbd{maximal factor perturbations under a fixed dataset \instance~so as to not change the explanation} (procedure: \emph{model training}). \krik{I think there is a subtle difference to counterfactual explanation that deserves thorough discussion in the related work section.}\amir{We can certainly have a related work section; does the second paragraph of \S2.2 capture the subtlety you have in mind?}

Our study reveals a surprising relationship between $E$ and $Y$ (precisely, measured by how a causal ancestor of the two influences them). 
In particular, for top-performing models, the influence on $E$ from $Y$ \textit{decreases} compared to relatively lower-performing models. For some methods, a causal ancestor of both $Y$ and $E$ directly influences $E$ much more than $Y$, leaving $Y$'s influence on $E$ minimal, even though this ancestor, i.e, hyperparameter, should not inform the explanation of the model in any way. % (i.e., it is determined prior to training the model).
This finding was consistent across 30k pre-trained models with different hyperparameters across different datasets.
%(SVHN data set shows decreased influence at top 5\% models). 
%In particular 
%\amir{if we're doing this for non-CIFAR datasets, we should ask Simon to run the tests for us now!}.
%\beenk{yes please. I thought we already had all the data for svh mnist fashion mnist but I was wrong?}
%Even when we subdivide the models into an importance axis (i.e., performance) with a hope to see a pattern, there is no strong indication that $E$ and $Y$ are influenced by hyperparameters in similar way, both in terms of correlation or ranked correlations.
% \been{[write more about our findings]}
 %We hope our work informs practitioners who use interpretability methods for a concrete task (e.g., debugging). 
Our work informs practitioners on what different explanation methods can and cannot be used for: if one's goal is to find $E$ that is related to the prediction, $Y$, methods with little relationship between $E$ and $Y$ under our framework aren't the best choices. Our framework can also be used to drive the development of new methods by providing a quantitative metric.
 
 %, and other precautions that must be in place before they use explanations for decision making.
 %reveals that there are more factors influencing $E$ than the prediction, $Y$ alone informs
 %the lack of relationships %between E and Y is a concrete step towards informing 
 %practitioners what these explanations can and cannot be used for. 
 %\been{edit this more}



\begin{comment}

\been{I would make this intro more to the point. Namely, 1) we have lot of interpretability methods, many more are developed. Lots of regulatory pressure. 2) we don't really understand how they work. eg., sanity check work and many others. We don't even know if predictions play a role in explanation or not (cite suraj's work on rethinking gradients). 3) this work, our main goal is to study the relationship between how a design decision/factors (e.g., choice of optimizers) that influences prediction v.s., explanation. In other words, will factors that influence prediction equally influence explanations? Viewed through a lens of causality.. [continue with your paragraph]}

\krik{(Following from what Been suggested): ``Since conducting experimental studies on all possible factors is too computationally prohibitive, we instead conduct observational studies on existing \emph{model zoos} and leverage tools from causal inference to draw our conclusions.''}

The field of \emph{explainable AI} (XAI) can be broadly split into two categories: \emph{inherent} and \emph{post-hoc} explainability~\citep{lipton2018mythos}.
%
The former is concerned with designing models that are interpretable by design\footnote{E.g., logistic regression, relatively shallow decision trees.}, whereas the latter is focused on the interpretation of a given (black-box) model.
%
In post-hoc explainability, it is assumed that the data and the model for which explanations are sought is given, which obfuscates any details about data pre-processing, the model training, and/or the interplay thereof.
%
% (e.g., interplay of hyperparameters).
%
We conjecture that such \emph{factors} (e.g., hyperparameters; \hparams~or $h$ for short) may have an effect (desirable or otherwise) on the resulting explanations, motivating the present study.
%
% which warrants the present study.

A careful study of the factors that play a role in generating outcomes is warranted, not just for XAI, but more generally in ML.
%
Earlier work has shown that models trained on completely different \hparams~could perform similarly under some metric (e.g., training loss), but have completely different task-specific performance (e.g., fairness)~\citep{d2020underspecification} which may be attributed to the seemingly benign but consequential randomization seed.
%
In the XAI literature specifically, prior work has shown that various saliency-based methods are independent of both the model and the underlying data, rendering the method unreliable~\citep{adebayo2018sanity, kindermans2019reliability}.



Building on previous work that identified cases of failure for such methods, our work sets out to quantify the effect of commonly overlooked factors (e.g., training \hparams) on the target explanations generated for ML models.
%
To do so, we consider the explanation generating process in \Cref{fig:pipeline_detail} and evaluate counterfactual queries of the form \emph{``had the training \hparams~taken on value $h'$ instead of $h$, would the explanation have been the same?''}\footnote{Because the world dynamics are stationary, this query yields the same answer as ``were the training \hparams~to take on value $h'$ instead of $h$, would the explanation remain the same?''}
%
Viewed through a len of causality, the counterfactual antecedent (i.e., \hparams~taking on value $h'$ as opposed to $h$) is a hypothetical intervention whose effect we want to measure on the target ($Y$ and $E$), conditioned on a particular instance, $x$, or subspace of the dataset, $\mathcal{X}' \subseteq \mathcal{X}$ (e.g., all dog images).\krik{It is unclear whether we only hold the data constant. How about other factors?  I guess we require a ``\emph{Ceteris paribus: other things held constant}'': }\amir{My understanding is that for ITE evaluation, we hold the instance fixed, but also all inter-\hparam~relations (all else being equal means all potentially causal relations, whatever is assumed).}
%
Essentially, we measure the \emph{treatment effect} of \hparams~on the down-stream explanations, for either an individual \instance~(ITE) and/or averaged over a population (ATE).
\krik{My suggestion: ``By treating \hparams~as a treatment and down-stream explanation as an outcome, we adopt the potential outcome framework [REFS: Rubin] to study the \emph{treatment effect} of \hparams~on different explanations. We consider treatment effects at both individual and population levels via an individual treatment effect (ITE) and average treatment effect (ATE), respectively.''}\amir{Very nice, will adopt, thanks!}
%
In the sections that follow, we formally introduce these concepts and describe how to compute them under varying computational budgets.

The application of causal inference in XAI has also guided other recent work~\citep{goyal2019explaining, zhao2021causal, karimi2020survey, karimi2020algorithmic, watson2021local, sani2020explaining, schwab2019cxplain}.
%
% An astute reader may notice that...
In fact, evaluating the treatment effects above bears a resemblance to another common explainability method, namely \emph{counterfactual explanations}~\citep{wachter2017counterfactual}.
%
This parallel is evident when thinking of \Cref{fig:pipeline_detail} in a coarser manner, i.e., $\mathcal{H},\mathcal{X} \rightarrow \mathcal{Y}/\mathcal{E}$, whereby the \hparams~and dataset \instance~enter a \emph{potentially blackbox but computable procedure} to yield a prediction and explanation. % (e.g., a classifier, a training pipeline)
%
% Whereas the counterfactual explanations of \citet{wachter2017counterfactual} are generated by perturbing the features of the dataset instance while holding the model fixed (i.e., the \hparams~do not change), evaluating \cref{eq:ite} in the present work perturbs the \hparams~on a fixed dataset instance.
Whereas the counterfactual explanations of \citet{wachter2017counterfactual} aim to identify minimal feature perturbations of the dataset \instance~under a fixed model to flip the prediction (i.e., \hparams~do not change; procedure: \emph{model prediction}), evaluating treatment effects as the difference between counterfactual contrasts is done to identify \tbd{maximal factor perturbations under a fixed dataset \instance~so as to not change the explanation} (procedure: \emph{model training}). \krik{I think there is a subtle difference to counterfactual explanation that deserves thorough discussion in the related work section.}\amir{We can certainly have a related work section; does the second paragraph of \S2.2 capture the subtlety you have in mind?}
\been{Putting the nuance in 2.2 makes more sense to me then having along intro}
% given under a fixed classifier where the hypothetical antecedent changes the features.

\been{This section likely to be shortened or removed?}
Although the aim of our work is to quantify the effect of often overlooked factors on generated explanations, we avoid making a claim as to whether or not, and to what extent, various factors should affect the outcome.
%
A major challenge in XAI is that explanations are deemed useful within application-specific or stakeholder-specific contexts, and therefore, universally ``good'' explanations are unattainable~\citep{doshi2017towards}.
%
Even in a specific context, the dearth of ground truth explanations makes it such that the quality of an explanation cannot be measured as its similarity to a canonical example, \tbd{but perhaps instead through a measure of stability or insensitivity/invariance to changes in unwanted factors/\hparams.}
%
\been{likely we can't really say "many" hparam set up? As readers might be imaging thousands of setups.}
By iterating over sufficiently many \hparam~setups and then generating and comparing the resulting explanations, one can evaluate the robustness of an explanation method to such factors.
%
% Variability of counterfactuals
% Variability of explanations across different settings is itself interesting, even if we can’t yet quantify it.
%
For instance, knowing that if the choice of optimizer changes, the explanation would focus on a dog’s feet instead of a dog’s ears is important.
%
In this regard, the present work can also be seen as an addition to the study of robustness of explanation.
%
\been{likely to be careful with claims regarding robustness! Might be opening a jar of worms for those reviewers who are allergic to robustness.}
Unlike earlier works which focused on the robustness of explanations to perturbations on input pixels~\citep{alvarez2018robustness, kindermans2019reliability, dombrowski2019explanations, yeh2019fidelity}, our work investigates how explanations change relative to changes in \hparams~via causally grounded treatment effects.
%
% Therefore, our contribution should be viewed as a method to quantify the importance \hl{(??)} of overlooked factors on generated explanations for the purpose of a deferred evaluation within each context.



% % In machine learning, unlike the task of prediction (classification or regression), explanation is an unsupervised learning problem.
% %
% It is generally accepted that explanations are defined within application-specific or stakeholder specific contexts, and that universally ``good'' explanations are unattainable, in part due to the dearth of ground truth explanations.
% %
% Therefore, we avoid making a claim as to whether or not, and to what extent, various factors should affect the output.
% %


% One challenge in XAI, the quality of an explanation cannot be measured as its similarity to a canonical example, but perhaps instead through a measure of stability or insensitivity/invariance to changes in unwanted factors/hyperparameters.
% %
% % By evaluating query \eqref{eq:counterfactual_explanation}
% By iterating over sufficiently many \hparam~setups and then generating and comparing the resulting explanations, one can evaluate the robustness of an explanation method to such factors.
% %
% % Variability of counterfactuals
% Variability of explanations across different settings is itself interesting, even if we can’t yet quantify it.
% %
% For instance, knowing that if the amount of regularization $\lambda$ changes, the explanation would focus on a dog’s feet instead of a dog’s ears is important.
% %

% % Due to our mechanical setup, a number of interesting observations arise.

\end{comment}


==> _sections/checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\small
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Please see \Cref{sec:analysis}.}
  \item Did you describe the limitations of your work?
    \answerYes{Please see limitation subsection in \Cref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The problem under investigation in our work is that of explaining ML explanations, as in what factors affect explanations, to what extend, and whether such effects co-occur for model predictions. At a high level, we quantitatively show that although some mutual effects of hyperparameters on $Y$ and $E$ can be observed, this relationship is not generally strong enough to warrant the unhinged deployment of existing explainability methods. In this regard, our work directly studies, and prescribes caution when using such methods to prevent potentially misleading results from explainability methods used for trust. Another noteworthy aspect of our work is the manner in which this investigation was undertaken. In particular, instead of utilizing many GPUs to train models under diverse hyperparameter settings, we employ a zoo of pretrained models, this saving on potential harms of large-scale training on the environment.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have read the ethics review guidelines and abide by those described on the NeurIPS website.}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{Please see \Cref{asp:exchangeability} and \Cref{asp:unconfoundedness}.}
  \item Did you include complete proofs of all theoretical results?
    \answerNA{Our manuscript is primarily empirical and contains to proofs.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Our code, preprocessing steps, and analysis framework will be open-sourced.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{We used an open-source zoo of pretrained models as described in \Cref{sec:methodology}; the corresponding paper is referenced and our analysis code will be released.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report error bars for correlation plots (confidence interval computed over different hyperparameters). Additionally, the violin plots show a distribution over the results. We omitted error bars from scatter plots, but instead summarize them in the aforementioned correlation plots.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    % \answerYes{Please see \Cref{sec:computational_details}.}
    \answerYes{We have used approximately 18,000 CPU core-hours. We used no GPUs for our analysis above.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Please see~\citep{unterthiner2020predicting} referenced throughout the text.}
  \item Did you mention the license of the assets?
    \answerYes{Although not mentioned in the main text due to lack of space, the repository from which the data was gathered (and where the corresponding license is mentioned) is appended to the bibliography entry.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
\normalsize

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> _sections/pipeline_coarse.tex <==
\begin{figure}[t]
  \centering
      \begin{tikzpicture}
        % x node set with absolute coordinates
        \node[det] (h) at (0,0) {$H$};
        \node[det] (x) [below = 0.6 cm of h] {$X$};
        \node[state] (y) [below right = 0.2 cm and 0.8 cm of h] {$Y$};
        \node[state] (e) [right = 0.6 cm of y] {$E$};
        
        % Directed edge
        \path (h) edge (y);
        \path (x) edge (y);
        \path (y) edge (e);
        \path (h) edge [bend left  = 25] (e);
        \path (x) edge [bend right = 25] (e);
      \end{tikzpicture}
%   \begin{subfigure}[c]{.35\linewidth}
%     \begin{center}
%       \begin{tikzpicture}
%         % x node set with absolute coordinates
%         \node[det] (h) at (0,0) {$H$};
%         % \node[state] (f) [right = 0.8 cm of h] {$F$};
%         \node[det] (x) [below = 0.8 cm of h] {$X$};
%         \node[state] (y) [below right=of h] {$Y$};
%         \node[state] (e) [right = 0.6 cm of y] {$E$};
        
%         % Directed edge
%         % \path (h) edge (f);
%         % \path (f) edge (y);
%         \path (h) edge (y);
%         \path (x) edge (y);
%         \path (y) edge (e);
%         % \path (h) edge [bend left  = 40] (e);
%         \path (f) edge [bend left  = 35] (e);
%         \path (x) edge [bend right = 20] (e);
%       \end{tikzpicture}
%     \end{center}
%   \end{subfigure}%
%   \begin{subfigure}[c]{.35\linewidth}
%     \begin{center}
%       \[
%       \left.
%       \begin{aligned}
%         F &\coloneqq \mathtt{T}(H, D) \\
%         Y &\coloneqq \mathtt{P}(F, X) \\
%         E &\coloneqq \mathtt{E}(F, X, Y) \\ 
%       \end{aligned}
%       \right\} ~~ \mathcal{M} 
%       \]
%     \end{center}
%   \end{subfigure}
  \caption{
  A course representation of \Cref{fig:pipeline_detail}, highlighting how interventions on factors (e.g., $H$, $X$) allow for studying the treatment effect (i.e., causal influence) of factors on down-stream targets (i.e., $Y$, $E$).
  %
%   Left and right show the graphical and the structural equation representation of the explanation generating process, respectively.
  %
  Training hyperparameters $H$ affect $Y$ and $E$ through the model architecture and weights obtain through the procedures $\mathtt{T}$, $\mathtt{P}$, $\mathtt{E}$. While not necessarily available in closed-form, these procedures are executable via an iterative (black-box) procedure on a computer.
  %
%   \been{can we remove F from this graph since we don't use it in this paper? Instead, we are combining F and Y and use Y (last layer of F) as a proxy for both.}\amir{I initially drew the graph without F, but then added it to better mirror Fig 1 and to allow for visually showing the structural equations (procedures) on the right. I don't feel strongly about this, so happy to remove if you'd like.}
  Note the absence of noise variables; under a fixed random seed, the procedures above yield outputs deterministically.
 }
%   \vspace{-5mm}
  \label{fig:pipeline_coarse}
\end{figure}
